"Other-Play" for Zero-Shot Coordination

We consider the problem of zero-shot coordination - constructing AI agents that can coordinate with novel partners they have not seen before (e.g. humans). Standard Multi-Agent Reinforcement Learning (MARL) methods typically focus on the self-play (SP) setting where agents construct strategies by playing the game with themselves repeatedly. Unfortunately, applying SP naively to the zero-shot coordination problem can produce agents that establish highly specialized conventions that do not carry over to novel partners they have not been trained with. We introduce a novel learning algorithm called other-play (OP), that enhances self-play by looking for more robust strategies, exploiting the presence of known symmetries in the underlying problem. We characterize OP theoretically as well as experimentally. We study the cooperative card game Hanabi and show that OP agents achieve higher scores when paired with independently trained agents. In preliminary results we also show that our OP agents obtains higher average scores when paired with human players, compared to state-of-the-art SP agents.

==> comments.tex <==
%% Example usage:
%\input{comments.tex}
%\commentstrue
%\setupcomments{ac}{Critch}{red!80!black}{color=red!30}
%\setupcomments{lc}{Lawrence}{green!70!black}{color=green!10}
%\setupcomments{sg}{Scott}{\red}{color=red!30}
%\setupcomments{ns}{Nate}{cyan}{color=cyan!30}
%\setupcomments{rb}{Robby}{yellow!40!black}{color=yellow!30}
%\setupcomments{se}{Sam}{\color{brown}}{color=brown!30}
%% predefined colors: black, blue, brown, cyan, darkgray, gray, green, lightgray, lime, magenta, olive, orange, pink, purple, red, teal, violet, white, yellow.

%%%%%%%%%%%%%

\usepackage{todonotes}
% Package needed for strikethrough:
\usepackage{soul}
% Package needed to avoid awful "Float(s) lost" errors
\usepackage{marginnote} % 

% Boolean toggling off the display of colored comments: 
\newif\ifcomments 

%Detects if a comment is being used in a footnote; without this, "Float(s) lost" errors will occur and be very difficult to find:
\newif\iffootnote
\let\Footnote\footnote
\renewcommand\footnote[1]{\begingroup\footnotetrue\Footnote{#1}\endgroup}

% Macro for setting up colored in-document comments:
\newcommand\setupcomments[4]{%%
\expandafter\def\csname#1says\endcsname##1{\ifcomments{\color{#3}\# #2 says: ##1 \#}\fi}%%
\expandafter\def\csname#1predicts\endcsname##1{\ifcomments{\color{#3}\# #2 predicts: ##1 \#}\fi}%%
\expandafter\def\csname#1adds\endcsname##1{\ifcomments{\color{#3} ##1}\fi}%%
\expandafter\def\csname#1rems\endcsname##1{\ifcomments{\color{#3} \st{##1}}\fi}
  \expandafter\def\csname#1box\endcsname##1{\ifcomments\vspace{1ex}\todo[inline,#4]{#2 says: ##1}{}\fi}%%

% Margin comments do not work in beamer:
  \expandafter\def\csname#1margin\endcsname##1{\ifcomments\marginnote{\todo[inline,#4]{#2 says: ##1}{}}\fi}%%
  \expandafter\def\csname#1section\endcsname##1{\ifcomments\todo[#4]{#2 says: ##1}{}\fi}%%
  \expandafter\def\csname#1todo\endcsname##1{\ifcomments\marginnote{\todo[inline]{#2 says: TODO: ##1}{}}\fi}%%

% Demo for new author

  \expandafter\def\csname#1demo\endcsname{\ifcomments
\noindent
$\backslash$#1says $\to$ \csname#1says\endcsname{example inline comment from #2.}\\
$\backslash$#1adds $\to$ \csname#1adds\endcsname{example addition by #2.}\\
$\backslash$#1rems $\to$ \csname#1rems\endcsname{example removal by #2.}\\
$\backslash$#1box $\to$ 
    \csname#1box\endcsname{example box comment from #2}
\fi}%%




}

%\renewcommand{\todo}[1]{\PackageError{Critch says:}{don't use \ todo; use \ xxtodo or \ xxmargin instead; \ todo can create impossible to find ``Float(s) lost" errors.}}

\commentstrue
